The ThreeDWorld Transport Challenge: A Visually Guided Task-and-Motion Planning Benchmark for Physically Realistic Embodied AI

We introduce a visually-guided and physics-driven task-and-motion planning benchmark, which we call the ThreeDWorld Transport Challenge. In this challenge, an embodied agent equipped with two 9-DOF articulated arms is spawned randomly in a simulated physical home environment. The agent is required to find a small set of objects scattered around the house, pick them up, and transport them to a desired final location. We also position containers around the house that can be used as tools to assist with transporting objects efficiently. To complete the task, an embodied agent must plan a sequence of actions to change the state of a large number of objects in the face of realistic physical constraints. We build this benchmark challenge using the ThreeDWorld simulation: a virtual 3D environment where all objects respond to physics, and where can be controlled using fully physics-driven navigation and interaction API. We evaluate several existing agents on this benchmark. Experimental results suggest that: 1) a pure RL model struggles on this challenge; 2) hierarchical planning-based agents can transport some objects but still far from solving this task. We anticipate that this benchmark will empower researchers to develop more intelligent physics-driven robots for the physical world.

==> api_table.tex <==
\begin{table*}[h]
\small
	\caption{Complete high-level API for the TDW Transport Challenge.}
	\label{tab:api}
	\begin{center}
		\begin{tabular}{l|p{3cm}|p{8cm}}
	\hline
			\textbf{Command Type}  &  \textbf{Command Name} & \textbf{Description} \\
	\hline
			Navigation  &  move\_to() & Move the agent to a target position or object.\\
	\hline
			Navigation & move\_by() & Move the agent forward by a distance along the agent's current forward directional vector.\\
	\hline
			Navigation & turn\_to() & Turn the agent to face a target position or object.\\
	\hline
			Navigation &  turn\_by() & Turn the agent by an angle.\\
	\hline
			Arm Articulation &  reach\_for() & Bend the arm joints of an agent to reach for a target position.\\
	\hline
			Arm Articulation &  grasp() & Grasp a target object.\\
\hline
			Arm Articulation &  pick\_up() & Grasp an object and lift it up. This combines the actions grasp() and reset\_arm().\\
	\hline
			Arm Articulation &  put\_in() & Try to put an object in a container.\\
    \hline
			Arm Articulation &  pour\_out() & Pour out all of the objects in a container held by one of the Magnebot's magnets.\\
	\hline
			Arm Articulation &  drop() & Drop an object held by the arm.\\
	\hline
			Arm Articulation &  reset\_arm() & Reset an agent's arm to its neutral position.\\
	\hline
			Scene Setup &  init\_scene() & Initialize a scene, populate it with objects, and add the agent.\\
	\hline
			Camera &  rotate\_camera() & Rotate an agent's camera around each axis.\\
    \hline
			Camera &  reset\_camera() & Reset the camera to its neutral position.\\
	\hline
			Camera &  add\_camera() & Add an overhead third-person camera to the scene.\\
	\hline
			Misc. &  get\_occupancy\_position() & Converts the position (i, j) in the occupancy map to (x, z) coordinates.\\
	\hline
			Misc. &  get\_visible\_objects() & Returns a list of visible objects.\\
	\hline
			Misc. &  end() & End the simulation.\\
	\hline

		\end{tabular}
		
		
	\end{center}


	\vspace{-6mm}	

	\end{table*}
